Linear-DPO: Linear Direct Preference Optimization for Diffusion and Flow-Matching Generative Models

Direct Preference Optimization (DPO) is successful for alignment in LLMs but still faces challenges in text-to-image generation. Existing studies are confined to denoising diffusion models while overlooking flow-matching, and suffer from an objective mismatch when applying discrete NLP-based DPO to regression-based generative tasks.\ In this paper, we derive a generalized DPO objective that covers both diffusion and flow-matching via a unified reverse-time SDE framework, and point out from a gradient perspective that the standard DPO objective is suboptimal for text-to-image generation. Consequently, we propose Linear-DPO, which replaces the aggressive sigmoid-based utility function with a sustained linear utility and incorporates an EMA-updated reference model. Qualitative and quantitative experiments on diffusion models (SD1.5, SDXL) and flow-matching model (SD3-Medium) demonstrate the superiority of our approach over existing baselines.

==> figure_sdxl.tex <==
\begin{figure}[bp]
  \centering
  % 1. 整体缩放到 80% 
  \begin{minipage}{0.9\textwidth}
    \fontfamily{ptm}\selectfont % 局部新罗马
    \setkeys{Gin}{width=\linewidth} % 图片宽度自适应
    
    % --- 第二行：SDXL ---
    \begin{minipage}[c]{0.03\linewidth}\rotatebox{90}{\textbf{ SDXL}}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_47_sdxl.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_24_sdxl.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_142_sdxl.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_158_sdxl.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_14_sdxl.jpg}\end{minipage}

    % --- 第三行：SFT ---
    \begin{minipage}[c]{0.03\linewidth}\rotatebox{90}{\textbf{SFT}}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_47_sdxl_sft.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_24_sdxl_sft.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_142_sdxl_sft.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_158_sdxl_sft.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_14_sdxl_sft.jpg}\end{minipage}

    % --- 第四行：Diffusion-DPO (简写为 DPO) ---
    \begin{minipage}[c]{0.03\linewidth}\rotatebox{90}{\textbf{ Diffusion-DPO}}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_47_sdxl_ddpo.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_24_sdxl_dpo.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_142_sdxl_dpo.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_158_sdxl_dpo.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_14_sdxl_dpo.jpg}\end{minipage}

    % --- 第五行：MaPO ---
    \begin{minipage}[c]{0.03\linewidth}\rotatebox{90}{\textbf{ MaPO}}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_47_sdxl_mapo.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_24_sdxl_mapo.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_142_sdxl_mapo.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_158_sdxl_mapo.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_14_sdxl_mapo.jpg}\end{minipage}

    % --- 第六行：Linear-DPO ---
    \begin{minipage}[c]{0.03\linewidth}\rotatebox{90}{\textbf{ Linear-DPO}}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_47_sdxl_linear.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_24_sdxl_linear.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_142_sdxl_linear.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_158_sdxl_linear.jpg}\end{minipage}%
    \begin{minipage}[c]{0.194\linewidth}\includegraphics{figures/image_14_sdxl_linear.jpg}\end{minipage}

    \vspace{0.5em} 

\hspace{0.03\linewidth}\hfill
\begin{minipage}[t]{0.194\linewidth}
    \centering
    \begin{minipage}[t]{0.85\linewidth} % 嵌套一层 85% 宽度的盒子实现强制留白
        \centering\tiny the fox in the labyrinth, vivid opulent colors, vector art
    \end{minipage}
\end{minipage}\hfill
\begin{minipage}[t]{0.194\linewidth}
    \centering
    \begin{minipage}[t]{0.85\linewidth}
        \centering\tiny a papaya fruit dressed as a sailor.
    \end{minipage}
\end{minipage}\hfill
\begin{minipage}[t]{0.194\linewidth}
    \centering
    \begin{minipage}[t]{0.95\linewidth} % 长 Prompt 留白稍小一点，防止行数过多
        % 针对极长 Prompt 缩小字号到 4.5pt
        \centering\fontsize{3.8pt}{5.4pt}\selectfont A warrior in glowing azure plate armor stands in a doorway to hell sliced by iridescent glass cracks, with crimson clouds and an art deco palace backdrop.
    \end{minipage}
\end{minipage}\hfill
\begin{minipage}[t]{0.194\linewidth}
    \centering
    \begin{minipage}[t]{0.95\linewidth}
        \centering\fontsize{5.5pt}{5.4pt}\selectfont The image depicts a stunning supernova within a fantasy artwork on Artstation.
    \end{minipage}
\end{minipage}\hfill
\begin{minipage}[t]{0.194\linewidth}
    \centering
    \begin{minipage}{0.95\linewidth}
        \centering\tiny motion
    \end{minipage}
\end{minipage}

  \end{minipage}
  \caption{Image samples generated from SDXL fine-tuned with various methods, using validation prompts from Pick-a-Pic v2, HPDv2 and PartiPrompt.}
\end{figure}
